Gleaning gravitational amplitudes -- a double copy for canceling dilatons

Scattering amplitudes in general relativity can be conveniently computed using the double copy, which relates them to Yang-Mills amplitudes. However, unwanted dilatons are sourced by massive scalar matter, which must be removed from the double copy in order to match the long range gravitational interactions. In this paper, we study how to automatically cancel out the dilatons by finding a suitable double-copy prescription in terms of gauge-theory fields, effectively treating the new contributions as ghosts that subtract out the unwanted states. At tree level, we find that an asymmetric double copy can reproduce the dilaton graphs in general dimension, which we explicitly verify up to six external massive scalars. Considering a one-loop four-point example, the same asymmetric double copy needs to be supplemented by the subtraction of bubble graphs that originate both from the axion and a residual dilaton term.

==> old_stuff.tex <==
%From the topologies we see that the Higgs particle flows between $k_{ab}$ and $k_{cd}$ in $g_1$, and between $k_{ab}$ and $k_{cd}$ and $k_{cd}$ and $k_{ef}$ in $g_2$. Because the expressions will be related via the Jacobi relations in Equation~\ref{eq:sixpoint jacobi}, we therefore choose an overall factor of $\mu_{ab} \cdot \mu_{cd}$ in both expressions,
% \begin{equation}
%     \mathfrak{A}^{6-point} = (\mu_{ab} \cdot \mu_{cd}) \Big( \alpha_1 (\varepsilon_a \cdot \varepsilon_b )(\varepsilon_c \cdot \varepsilon_d)(\varepsilon_e \cdot \varepsilon_f)(a \cdot b) +...+\alpha_{900} (\varepsilon _a\cdot \varepsilon _d)( \varepsilon _b\cdot \varepsilon _c)  (k_b\cdot \varepsilon _e)( k_b\cdot \varepsilon _f)
%     \Big),
% \end{equation}


\subsection{Old subtle cut}
The third cut is more subtle, and we will therefore give the full expression
\begin{equation}
\begin{aligned}
    g_2^{\mathfrak{MC}} =& 
    \begin{gathered}
    \begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.4, 0.6) {\(c\)};
\vertex (c2) at (0.4, 0.6) {\(d\)};
\vertex (cut11) at (-0.45, 0.3);
\vertex (cut12) at (-0.45, -0.3);
\vertex (cut21) at (0.45, 0.3);
\vertex (cut22) at (0.45, -0.3);
\vertex (cut31) at (0,0.3);
\vertex (cut32) at (0,-0.3);
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[dashed] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[dashed](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c1),
(mid21) --[thick, green(ncs)] (c2),
(cut11) --[color=red,thick, dashed] (cut12),
(cut21) --[color=red,thick, dashed] (cut22),
(cut31) --[color=red,thick, dashed] (cut32)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    \\
    =&  ( \mu _a\cdot \mu _c) ( \mu _c\cdot \mu _e )(\varepsilon _a\cdot \varepsilon _b)( \varepsilon _c\cdot \varepsilon _d)(\varepsilon _e\cdot \varepsilon _f)
    \\
   & + ( \mu _a\cdot \mu _c)( \mu _c\cdot \mu _e)
   (\varepsilon _a\cdot \varepsilon _b)( \varepsilon _e\cdot \varepsilon _f )
    \frac{ \left(k_a\cdot \varepsilon _c+k_b\cdot \varepsilon _c\right) \left(k_e\cdot \varepsilon _d+k_f\cdot \varepsilon _d\right)}{\mu _c^2}
    \end{aligned}.
\end{equation}
Here we will make a similar simplification as the four-point amplitude with two external Higgs particles, where remembering that the masses $\mu_i$ are scalar components we rearrange, 
\begin{equation}
    ( \mu _a\cdot \mu _c)( \mu _c\cdot \mu _e) \to \mu^2_c ( \mu _a\cdot \mu _e),
\end{equation}
so that the cut expression $g_2^{\mathfrak{MC}}$ becomes, 
\begin{equation}
g_2^{\mathfrak{MC}} = 
(\mu _a\cdot \mu _e)
(\varepsilon _a\cdot \varepsilon _b)  (\varepsilon _e\cdot \varepsilon _f) \left(\left(k_e\cdot \varepsilon _d+k_f\cdot \varepsilon _d\right) \left(k_a\cdot \varepsilon _c+k_b\cdot \varepsilon _c\right)+\mu_c^2 ~\varepsilon _c\cdot \varepsilon _d\right).
\end{equation}
After this rearrangement the maximal cuts obey the Jacobi relations in Equation~\ref{eq:sixpoint jacobi}, and the resulting cuts constrain a further 301 coefficients, leaving a total of 17 undetermined coefficients. The next step is to compare with the maximal and next-to-maximal cuts of the massive scalars coupled to gravity amplitudes.

% All four-point amplitudes in one figure
\begin{figure}
\centering
\begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1, -0.5) {\(1\)};
\vertex (a2) at (-1, 0.5) {\(2\)};
\vertex (mid1) at (-0.3,0);
\vertex (mid2) at (0.3,0);
\vertex (b1) at (1, -0.5) {\(4\)};
\vertex (b2) at (1, 0.5) {\(3\)};
\diagram{
(a1)--[thick, red] (mid1),
(a2) -- [thick, red] (mid1),
(mid1)--[gluon](mid2), 
(mid2) --[thick, blue(ncs)] {(b1), (b2)}
};
\end{feynman}
\end{tikzpicture}
~
\begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1, -0.5) {\(1\)};
\vertex (a2) at (-1, 0.5) {\(2\)};
\vertex (mid1) at (-0.3,0);
\vertex (mid2) at (0.3,0);
\vertex (b1) at (1, -0.5) {\(4\)};
\vertex (b2) at (1, 0.5) {\(3\)};
\diagram{
(a1)--[thick, red] (mid1),
(a2) -- [thick, red] (mid1),
(mid1)--[dashed](mid2), 
(mid2) --[thick, blue(ncs)] {(b1), (b2)}
};
\end{feynman}
\end{tikzpicture}
 ~
\begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1, -0.5) {\(1\)};
\vertex (a2) at (-1, 0.5) {\(2\)};
\vertex (mid1) at (-0.3,0);
\vertex (mid2) at (0.3,0);
\vertex (b1) at (1, -0.5) {\(4\)};
\vertex (b2) at (1, 0.5) {\(3\)};
\diagram{
(a1)--[thick, red] (mid1),
(a2) -- [thick, red] (mid1),
(mid1)--[gluon](mid2), 
(mid2) --[dashed] {(b1), (b2)}
};
\end{feynman}
\end{tikzpicture}
\\
\begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1, -0.5) {\(1\)};
\vertex (a2) at (-1, 0.5) {\(2\)};
\vertex (mid1) at (-0.3,0);
\vertex (mid2) at (0.3,0);
\vertex (b1) at (1, -0.5) {\(4\)};
\vertex (b2) at (1, 0.5) {\(3\)};
\diagram{
(a1)--[thick, red] (mid1),
(a2) -- [thick, red] (mid1),
(mid1)--[dashed](mid2), 
(mid2) --[dashed] (b1),
(mid2) --[gluon] (b2)
};
\end{feynman}
\end{tikzpicture}
~
\begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1, -0.5) {\(1\)};
\vertex (a2) at (-1, 0.5) {\(2\)};
\vertex (mid1) at (-0.3,0);
\vertex (mid2) at (0.3,0);
\vertex (b1) at (1, -0.5) {\(4\)};
\vertex (b2) at (1, 0.5) {\(3\)};
\diagram{
(a1)--[dashed] (mid1),
(a2) -- [dashed] (mid1),
(mid1)--[gluon](mid2), 
(mid2) --[dashed] {(b1), (b2)}
};
\end{feynman}
\end{tikzpicture}
~
\begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1, -0.5) {\(1\)};
\vertex (a2) at (-1, 0.5) {\(2\)};
\vertex (mid1) at (-0.3,0);
\vertex (mid2) at (0.3,0);
\vertex (b1) at (1, -0.5) {\(4\)};
\vertex (b2) at (1, 0.5) {\(3\)};
\diagram{
(a1)--[dashed] (mid1),
(a2) -- [dashed] (mid1),
(mid1)--[gluon](mid2), 
(mid2) --[gluon] {(b1), (b2)}
};
\end{feynman}
\end{tikzpicture}
\caption{Four-point amplitudes (represented by one graph from each amplitude).}
\label{Tab: 1 massive scalar trees dilatons}
\end{figure}

\iffalse
\begin{equation}
A_4(k_1, k_2, k_3, k_4) :
     \begin{gathered}
    \begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1, -0.5) {\(1\)};
\vertex (a2) at (-1, 0.5) {\(2\)};
\vertex (mid1) at (-0.3,0);
\vertex (mid2) at (0.3,0);
\vertex (b1) at (1, -0.5) {\(4\)};
\vertex (b2) at (1, 0.5) {\(3\)};
\diagram{
{(a1), (a2)}--[dashed] (mid1),
(mid1) --[gluon] (mid2),
(mid2) --[dashed] {(b1), (b2)}
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}.
\end{equation}
\fi

\iffalse
\begin{equation}
\mathfrak{C}_4^b =
    \begin{gathered}
    \begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1, -0.5) {\(1\)};
\vertex (a2) at (-1, 0.5) {\(2\)};
\vertex (mid1) at (-0.3,0);
\vertex (mid11) at (-0.05, 0);
\vertex (mid2) at (0.3,0);
\vertex (mid22) at (0.05, 0);
\vertex (b1) at (1, -0.5) {\(4\)};
\vertex (b2) at (1, 0.5) {\(3\)};
\vertex (c1) at (0, 0.6);
\vertex (c2) at (0,-0.6);
\diagram{
{(a1), (a2)}--[dashed] (mid1),
(mid1) --[gluon] (mid11),
(mid22) --[gluon] (mid2),
(mid2) --[dashed] {(b1), (b2)},
(c1) --[thick, color=red, dashed] (c2)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    = 
    \sum_{\text{states}}A^{HHg}_3(k_1, k_2, l)A_3^{HHg}(-l, k_3, k_4),
\end{equation}
\fi

\begin{equation}
\begin{aligned}
   g_6^{a1} =  
   \begin{gathered}
    \begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.4, 0.6) {\(c\)};
\vertex (c2) at (0.4, 0.6) {\(d\)};
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[dashed] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[photon](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c1),
(mid21) --[thick, green(ncs)] (c2)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    \hspace{0.3cm}
    ,
    \hspace{0.3cm}
g_6^{a2}=     
\begin{gathered}
    \begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.4, 0.6) {\(c\)};
\vertex (c2) at (0.4, 0.6) {\(d\)};
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[dashed] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[dashed](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c1),
(mid21) --[thick, green(ncs)] (c2)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered},\\
    g_6^{a3}
   = 
   \begin{gathered}
    \begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid2) at (0.6,0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.3, 0.9) {\(c\)};
\vertex (c2) at (0.3, 0.9) {\(d\)};
\vertex (midb) at (0,0);
\vertex (midt) at (0,0.4);
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[dashed](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(midb) -- [photon](midt),
(midt) --[thick, green(ncs)] {(c1), (c2)}
};
\end{feynman}
\end{tikzpicture}
    \end{gathered},
    \hspace{3cm}
    \end{aligned}
\end{equation}

\begin{align}
    \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid2) at (0.6,0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.3, 0.9) {\(c\)};
\vertex (c2) at (0.3, 0.9) {\(d\)};
\vertex (midb) at (0,0);
\vertex (midt) at (0,0.4);
\diagram{
{(a1), (a2)}--[thick, red] (mid1),
(mid1) --[dashed](midb),
(midb) --[photon](mid2),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(midb) -- [dashed](midt),
(midt) --[thick, green(ncs)] {(c1), (c2)}
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    &= 
     \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.4, 0.6) {\(c\)};
\vertex (c2) at (0.4, 0.6) {\(d\)};
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[dashed] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[photon](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c1),
(mid21) --[thick, green(ncs)] (c2)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    - 
     \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.4, 0.7) {\(c\)};
\vertex (c2) at (0.4, 0.7) {\(d\)};
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[dashed] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[photon](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c2),
(mid21) --[thick, green(ncs)] (c1)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    \\
  \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid2) at (0.6,0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.3, 0.9) {\(c\)};
\vertex (c2) at (0.3, 0.9) {\(d\)};
\vertex (midb) at (0,0);
\vertex (midt) at (0,0.4);
\diagram{
{(a1), (a2)}--[thick, red] (mid1),
(mid1) --[dashed](mid2),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(midb) -- [photon](midt),
(midt) --[thick, green(ncs)] {(c1), (c2)}
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    &=   f_D \left(
     \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.4, 0.6) {\(c\)};
\vertex (c2) at (0.4, 0.6) {\(d\)};
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[dashed] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[dashed](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c1),
(mid21) --[thick, green(ncs)] (c2)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    - 
     \begin{gathered}
    \begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.4, 0.7) {\(c\)};
\vertex (c2) at (0.4, 0.7) {\(d\)};
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[dashed] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[dashed](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c2),
(mid21) --[thick, green(ncs)] (c1)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    \right),
\end{align}

\begin{align}
    g_1^{\mathfrak{MC}} &= 
    \begin{gathered}
    \begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.4, 0.6) {\(c\)};
\vertex (c2) at (0.4, 0.6) {\(d\)};
\vertex (cut11) at (-0.45, 0.3);
\vertex (cut12) at (-0.45, -0.3);
\vertex (cut21) at (0.45, 0.3);
\vertex (cut22) at (0.45, -0.3);
\vertex (cut31) at (0,0.3);
\vertex (cut32) at (0,-0.3);
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[dashed] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[photon](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c1),
(mid21) --[thick, green(ncs)] (c2),
(cut11) --[color=red,thick, dashed] (cut12),
(cut21) --[color=red,thick, dashed] (cut22),
(cut31) --[color=red,thick, dashed] (cut32)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    = - (\mu _a\cdot \mu _c )(k_d\cdot k_f),
    \\
     g_3^{\mathfrak{MC}} &= 
     \begin{gathered}
    \begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid2) at (0.6,0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.3, 0.9) {\(c\)};
\vertex (c2) at (0.3, 0.9) {\(d\)};
\vertex (midb) at (0,0);
\vertex (midt) at (0,0.4);
\vertex (cut11) at (-0.45, 0.3);
\vertex (cut12) at (-0.45, -0.3);
\vertex (cut21) at (0.45, 0.3);
\vertex (cut22) at (0.45, -0.3);
\vertex (cut31) at (-0.25,0.2);
\vertex (cut32) at (0.25,0.2);
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[dashed](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(midb) -- [photon](midt),
(midt) --[thick, green(ncs)] {(c1), (c2)},
(cut11) --[color=red,thick, dashed] (cut12),
(cut21) --[color=red,thick, dashed] (cut22),
(cut31) --[dashed, thick, color=red] (cut32)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    = - (\mu _a\cdot \mu _e) \left(k_d\cdot k_e+k_d\cdot k_f\right),\\
    g_2^{\mathfrak{MC}} &= 
    \begin{gathered}
    \begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.4, 0.6) {\(c\)};
\vertex (c2) at (0.4, 0.6) {\(d\)};
\vertex (cut11) at (-0.45, 0.3);
\vertex (cut12) at (-0.45, -0.3);
\vertex (cut21) at (0.45, 0.3);
\vertex (cut22) at (0.45, -0.3);
\vertex (cut31) at (0,0.3);
\vertex (cut32) at (0,-0.3);
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[dashed] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[dashed](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c1),
(mid21) --[thick, green(ncs)] (c2),
(cut11) --[color=red,thick, dashed] (cut12),
(cut21) --[color=red,thick, dashed] (cut22),
(cut31) --[color=red,thick, dashed] (cut32)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    =  ( \mu _a\cdot \mu _c) ( \mu _c\cdot \mu _e ).
\end{align}

\begin{equation}
\begin{aligned}
     m_1^{\mathfrak{MC}} &= 
    \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.4, 0.6) {\(c\)};
\vertex (c2) at (0.4, 0.6) {\(d\)};
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[photon, thick] (mid11),
(mid11) --[photon, thick] (mid1),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[photon, thick](mid2),
(mid2)--[photon, thick](mid21),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c1),
(mid21) --[thick, green(ncs)] (c2)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}\\
    &= 
    \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.4, 0.6) {\(c\)};
\vertex (c2) at (0.4, 0.6) {\(d\)};
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[photon] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[ghost](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c1),
(mid21) --[thick, green(ncs)] (c2)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    +
    \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.4, 0.6) {\(c\)};
\vertex (c2) at (0.4, 0.6) {\(d\)};
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[ghost] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[photon](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c1),
(mid21) --[thick, green(ncs)] (c2)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    +
    \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.4, 0.6) {\(c\)};
\vertex (c2) at (0.4, 0.6) {\(d\)};
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[ghost] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[ghost](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c1),
(mid21) --[thick, green(ncs)] (c2)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered},
    \\
    &= 
    \mu _a^2\mu _c^2 \frac{ \left(k_d\cdot k_e\right){}^2}{D_s - 2}+
    \mu _e^2 \mu _c^2\frac{  \left(k_b\cdot k_f\right){}^2}{D_s - 2}-\frac{\mu _1^2 \mu _c^2 \mu _e^4}{(D_s - 2)^2},
\end{aligned}
\end{equation}

\begin{equation}
    \begin{aligned}
    m_2^{\mathfrak{MC}}
    &=
    \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid2) at (0.6,0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.3, 0.9) {\(c\)};
\vertex (c2) at (0.3, 0.9) {\(d\)};
\vertex (midb) at (0,0);
\vertex (midt) at (0,0.4);
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[thick, photon](mid2),
(mid2) --[thick, photon](mid1),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(midb) -- [photon, thick](midt),
(midt) -- [photon, thick](midb),
(midt) --[thick, green(ncs)] {(c1), (c2)}
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    \\
    &=
    \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid2) at (0.6,0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.3, 0.9) {\(c\)};
\vertex (c2) at (0.3, 0.9) {\(d\)};
\vertex (midb) at (0,0);
\vertex (midt) at (0,0.4);
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[ghost](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(midb) -- [photon](midt),
(midt) --[thick, green(ncs)] {(c1), (c2)}
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    +
     \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid2) at (0.6,0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.3, 0.9) {\(c\)};
\vertex (c2) at (0.3, 0.9) {\(d\)};
\vertex (midb) at (0,0);
\vertex (midt) at (0,0.4);
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[ghost](midb),
(midb) --[photon](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(midb) -- [ghost](midt),
(midt) --[thick, green(ncs)] {(c1), (c2)}
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
+
   \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid2) at (0.6,0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.3, 0.9) {\(c\)};
\vertex (c2) at (0.3, 0.9) {\(d\)};
\vertex (midb) at (0,0);
\vertex (midt) at (0,0.4);
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[photon](midb),
(midb) --[ghost](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(midb) -- [ghost](midt),
(midt) --[thick, green(ncs)] {(c1), (c2)}
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}\\
    &= \mu _a^2\mu _e^2 \frac{ \left(k_d\cdot k_e+k_d\cdot k_f\right){}^2}{D_s-2}
    +
    \mu _a^2\mu _c^2 \frac{ \left(k_c\cdot k_f+k_d\cdot k_f\right){}^2}{D_s-2}
    +
    \mu _c^2 \mu _e^2
    \frac{ \left(k_b\cdot k_e+k_b\cdot k_f\right){}^2}{D_s -2}
    .
    \end{aligned}
\end{equation}

\begin{equation}
    \begin{aligned}
    \mathfrak{C}^{N-Max}_1 &= 
    \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.4, 0.7) {\(c\)};
\vertex (c2) at (0.4, 0.7) {\(d\)};
\vertex[blob,label={ }] (m) at ( 0, 0) {\contour{ }};
\diagram{
{(a1), (a2)}--[thick, red] (mid1),
(mid1) --[photon, thick] (m),
(m) --[photon, thick] (mid1),
(m)--[photon, thick](mid2),
(mid2)--[photon, thick](m),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(m) --[thick, green(ncs)] (c1),
(m) --[thick, green(ncs)] (c2)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    \\
    &=
    \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.4, 0.6) {\(c\)};
\vertex (c2) at (0.4, 0.6) {\(d\)};
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[photon] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[ghost](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c1),
(mid21) --[thick, green(ncs)] (c2)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    +
    \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.4, 0.6) {\(c\)};
\vertex (c2) at (0.4, 0.6) {\(d\)};
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[ghost] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[photon](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c1),
(mid21) --[thick, green(ncs)] (c2)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    +
    \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.4, 0.6) {\(c\)};
\vertex (c2) at (0.4, 0.6) {\(d\)};
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[ghost] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[ghost](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c1),
(mid21) --[thick, green(ncs)] (c2)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    \\
&+
    \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.3, 0.6) {\(c\)};
\vertex (c2) at (0.3, 0.6) {\(d\)};
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[photon] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[ghost](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c2),
(mid21) --[thick, green(ncs)] (c1)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    +
    \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.3, 0.6) {\(c\)};
\vertex (c2) at (0.3, 0.6) {\(d\)};
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[ghost] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[photon](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c2),
(mid21) --[thick, green(ncs)] (c1)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    +
    \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid11) at (-0.2,0);
\vertex (mid2) at (0.6,0);
\vertex (mid21) at (0.2, 0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.3, 0.6) {\(c\)};
\vertex (c2) at (0.3, 0.6) {\(d\)};
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[ghost] (mid11),
(mid11) --[thick, green(ncs)] (mid21),
(mid21)--[ghost](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(mid11) --[thick, green(ncs)] (c2),
(mid21) --[thick, green(ncs)] (c1)
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    \\
    &+
    \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid2) at (0.6,0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.3, 0.9) {\(c\)};
\vertex (c2) at (0.3, 0.9) {\(d\)};
\vertex (midb) at (0,0);
\vertex (midt) at (0,0.4);
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[ghost](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(midb) -- [photon](midt),
(midt) --[thick, green(ncs)] {(c1), (c2)}
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
    +
     \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid2) at (0.6,0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.3, 0.9) {\(c\)};
\vertex (c2) at (0.3, 0.9) {\(d\)};
\vertex (midb) at (0,0);
\vertex (midt) at (0,0.4);
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[ghost](midb),
(midb) --[photon](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(midb) -- [ghost](midt),
(midt) --[thick, green(ncs)] {(c1), (c2)}
};
\end{feynman}
\end{tikzpicture}
    \end{gathered}
+
   \begin{gathered}
    \begin{tikzpicture}[scale=1.3]
\begin{feynman}
\vertex (a1) at (-1.3, -0.5) {\(a\)};
\vertex (a2) at (-1.3, 0.5) {\(b\)};
\vertex (mid1) at (-0.6,0);
\vertex (mid2) at (0.6,0);
\vertex (b1) at (1.3, -0.5) {\(f\)};
\vertex (b2) at (1.3, 0.5) {\(e\)};
\vertex (c1) at (-0.3, 0.9) {\(c\)};
\vertex (c2) at (0.3, 0.9) {\(d\)};
\vertex (midb) at (0,0);
\vertex (midt) at (0,0.4);
\diagram{
(a1)--[thick, red] (mid1),
(mid1) --[photon](midb),
(midb) --[ghost](mid2),
(a2) -- [thick, red] (mid1),
(mid2) --[thick, blue(ncs)] {(b1), (b2)},
(midb) -- [ghost](midt),
(midt) --[thick, green(ncs)] {(c1), (c2)}
};
\end{feynman}
\end{tikzpicture}
    \end{gathered},
    \\
=& \hspace{0.4cm}
\frac{1}{2\left(k_d\cdot k_e+k_d\cdot k_f\right)}
\left[ 
\frac{\mu _c^2 \mu _a^2 \left(k_d\cdot k_e\right){}^2}{D_s-2}
+
\frac{\mu _c^2 \mu _a^2 \left(k_d\cdot k_e\right){}^2}{D_s-2}
- 
\frac{\mu _a^2 \mu _c^4 \mu _e^2}{(D_s-2)^2}
\right]
\\
&+
\frac{1}{2 \left(k_c\cdot k_e+k_c\cdot k_f\right)}
\left[
\frac{\mu _c^2 \mu _e^2 \left(k_b\cdot k_d\right){}^2}{ (D_s-2) }
+
\frac{\mu _c^2\mu _e^2 \left(k_b\cdot k_d\right){}^2}{ (D_s-2) }-\frac{\mu _a^2 \mu _c^4 \mu _e^2}{ (D_s-2)^2 }
\right]
\\
&- \frac{1}{(k_c+k_d)^2}
\Bigg[
\frac{\mu _a^2\mu _c^2 \left(k_c\cdot k_e+k_d\cdot k_e\right){}^2}{D_s-2 }+\frac{\mu _a^2\mu _e^2 \left(k_c\cdot k_e+k_c\cdot k_f\right){}^2}{D_s-2}
\\
&\hspace{7cm}+\frac{\mu _c^2 \mu _e^2 \left(k_b\cdot k_e+k_b\cdot k_f\right){}^2}{D_s-2}
\Bigg]
\\
& +\frac{\mu _a^2 \mu _e^2 \left(k_c\cdot k_e+k_c\cdot k_f\right)}{2 (D_s-2)}-\frac{\mu _a^2 \mu _c^2 \mu _e^2}{(D_s-2)^2},
    \end{aligned}
\end{equation}

\iffalse
\begin{equation}
\begin{gathered}
\begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1, -0.5) {\(2\)};
\vertex (a2) at (-1, 0.5) {\(3\)};
\vertex (mid1) at (-0.3,0);
\vertex (mid2) at (0.5,0) {\(1\)};
\diagram{
(a1)--[gluon] (mid1),
(a2) -- [gluon] (mid1),
(mid1)--[gluon](mid2)
};
\end{feynman}
\end{tikzpicture}
\end{gathered}
\hspace{0.3cm}
\Rightarrow
\hspace{0.3cm}
    \begin{gathered}
\begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1, -0.5) {\(2\)};
\vertex (a2) at (-1, 0.5) {\(3\)};
\vertex (mid1) at (-0.3,0);
\vertex (mid2) at (0.5,0) {\(1\)};
\diagram{
(a1)--[thick, red] (mid1),
(a2) -- [thick, red] (mid1),
(mid1)--[gluon](mid2)
};
\end{feynman}
\end{tikzpicture}
\end{gathered}
+
 \begin{gathered}
\begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1, -0.5) {\(2\)};
\vertex (a2) at (-1, 0.5) {\(3\)};
\vertex (mid1) at (-0.3,0);
\vertex (mid2) at (0.5,0) {\(1\)};
\diagram{
(a1)--[thick, red] (mid1),
(a2) -- [thick, red] (mid1),
(mid1)--[dashed](mid2)
};
\end{feynman}
\end{tikzpicture}
\end{gathered}
+
\begin{gathered}
\begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1, -0.5) {\(2\)};
\vertex (a2) at (-1, 0.5) {\(3\)};
\vertex (mid1) at (-0.3,0);
\vertex (mid2) at (0.5,0) {\(1\)};
\diagram{
(a1)--[dashed] (mid1),
(a2) -- [dashed] (mid1),
(mid1)--[gluon](mid2)
};
\end{feynman}
\end{tikzpicture}
\end{gathered},
\end{equation}
\fi

\iffalse
\begin{equation}\label{Eq: 3-point Higgs}
\begin{gathered}
\begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1, -0.5) {\(2\)};
\vertex (a2) at (-1, 0.5) {\(3\)};
\vertex (mid1) at (-0.3,0);
\vertex (mid2) at (0.5,0) {\(1\)};
\diagram{
(a1)--[thick, red] (mid1),
(a2) -- [thick, red] (mid1),
(mid1)--[dashed](mid2)
};
\end{feynman}
\end{tikzpicture}
\end{gathered}
:
    A_{\text{Higgs}} =
   - (\mu _1\cdot \varepsilon _1)\left(\varepsilon _2\cdot \varepsilon _3\right) ,
\\
\end{equation}
\begin{equation}\label{Eq: 3-point Higgs gluon}
    \begin{gathered}
\begin{tikzpicture}[scale=1.5]
\begin{feynman}
\vertex (a1) at (-1, -0.5) {\(2\)};
\vertex (a2) at (-1, 0.5) {\(3\)};
\vertex (mid1) at (-0.3,0);
\vertex (mid2) at (0.5,0) {\(1\)};
\diagram{
(a1)--[dashed] (mid1),
(a2) -- [dashed] (mid1),
(mid1)--[gluon](mid2)
};
\end{feynman}
\end{tikzpicture}
\end{gathered}
:
A_{\text{Higgs+gluon}}
= 
( k_3\cdot \varepsilon_1)(\varepsilon _2\cdot \varepsilon _3),
\end{equation}
\fi

 \Ingrid{However, we encounter a problem when using the massive state projector in Equation~(something) to sew together massive legs. Previously, we remedied this by rewriting $(\mu_1 \cdot \varepsilon_1)(\mu \cdot \varepsilon_2) \leftarrow \mu^2~(\varepsilon_1 \cdot \varepsilon_2)$. While this allows for the Jacobi relation described in Section~(something), it also fixes the dimension $D_s$, and allowing a similar rewriting when sewing together a next-to-maximal cut allows information from the non-scalar part to bleed into the scalar part.} 
